A communication efficient distributed learning framework for smart environments

Due to the pervasive diffusion of personal mobile and IoT devices, many ``smart environments'' (e.g., smart cities and smart factories) will be, among others, generators of huge amounts of data. Currently, this is typically achieved through centralised cloud-based data analytics services. However, according to many studies, this approach may present significant issues from the standpoint of data ownership, and even wireless network capacity. One possibility to cope with these shortcomings is to move data analytics closer to where data is generated. In this paper, we tackle this issue by proposing and analyzing a distributed learning framework, whereby data analytics are performed at the edge of the network, i.e., on locations very close to where data is generated. Specifically, in our framework, partial data analytics are performed directly on the nodes that generate the data, or on nodes close by (e.g., some of the data generators can take this role on behalf of subsets of other nodes nearby). Then, nodes exchange partial models and refine them accordingly. Our framework is general enough to host different analytics services. In the specific case analysed in the paper, we focus on a learning task, considering two distributed learning algorithms. Using an activity recognition and a pattern recognition task, both on reference datasets, we compare the two learning algorithms between each other and with a central cloud solution (i.e., one that has access to the complete datasets). Our results show that using distributed machine learning techniques, it is possible to drastically reduce the network overhead, while obtaining performance comparable to the cloud solution in terms of learning accuracy. The analysis also shows when each distributed learning approach is preferable, based on the specific distribution of the data on the nodes.

==> problem.tex <==
\section{Problem statement and system assumptions}
\label{sec:statement}


%In this paper we assume that
%a dataset $D$ is distributed over different devices located in a number $L$ of
%different physical locations.  Therefore each location $l$ holds a partition
%$D_l, l=1,\dots,L$ of $D$. Clearly, we assume that the data contained in
%each partition $D_l$ are homogeneous, e.g., for a sensing application, they must
%be related to a well-defined physical entity that is sensed across different
%locations. This is necessary to meaningfully use, for the
%model corresponding to one partition, features of the models trained on the rest
%of the partitions.
%
%In this paper we focus on supervised
%learning problems and more precisely, we consider a classification problem.
%Specifically, we assume that the partitions $D_l$ are the training sets for 
%training $l$ partial classifier, which are then refined based on each other
%features. Therefore, each local dataset is in the form $D_l =  \{\bf{X}_l,Y_l\}$ where
%$X_l\in\mathbb{R}^{n_l\times d}$ is the set of examples (or patterns) available
%at the $l$-th location $l$, $Y_l\in\mathbb{R}^{n_l\times 1}$ is the set of labels that
%define the class to which each pattern belongs to, $n_l$ is the cardinality of
%$D_l$ and $d$ is the number of features of each pattern $\bf{x}\in\bf{X}$ (i.e.,
%the dimensionality of each data point in the dataset).
%
%
%Our
%purpose is twofold. On the one hand we want that  at the end of the distributed
%learning process, each machine belonging to a location $l$ has learnt a model
%from its own data, with a prediction accuracy equivalent to the one obtainable
%in a cloud settings, i.e. the case when all data is accessible from the cloud
%and the learning process is accomplished considering the union of all the local
%datasets.  On the other hand we want to minimize the traffic load over the
%network. In this layout we consider the all that machines at different locations
%can communicate information between each others through the network but, they
%are not allowed to share their own datasets $D_l$. The only information that
%each machine is allowed to share with all the other machines is about the models
%they have learnt from their local dataset. %In this paper we will denote the
%model learnt in the location $l$ with $M_l$.   
%

